Building a Chinese Medical Dialogue System: Integrating Large-scale Corpora and Novel Models

The global COVID-19 pandemic underscored major deficiencies in traditional healthcare systems, hastening the advancement of online medical services, especially in medical triage and consultation. However, existing studies face two main challenges. First, the scarcity of large-scale, publicly available, domain-specific medical datasets due to privacy concerns, with current datasets being small and limited to a few diseases, limiting the effectiveness of triage methods based on Pre-trained Language Models (PLMs). Second, existing methods lack medical knowledge and struggle to accurately understand professional terms and expressions in patient-doctor consultations. To overcome these obstacles, we construct the Large-scale Chinese Medical Dialogue Corpora (LCMDC), thereby addressing the data shortage in this field. Moreover, we further propose a novel triage system that combines BERT-based supervised learning with prompt learning, as well as a GPT-based medical consultation model. To enhance domain knowledge acquisition, we pre-trained PLMs using our self-constructed background corpus. Experimental results on the LCMDC demonstrate the efficacy of our proposed systems.

==> 7-discussion.tex <==
\section{Discussion and Future Work}

We discuss the biases in online medical data, AI adoption in healthcare, and the development of large language models in different sectors. For details, please refer to Appendix~\ref{app:diss}.

Looking ahead, future work focuses on expanding datasets to reduce bias, enhancing intelligent triage systems with background knowledge and multi-modal methods, and refining medical consultation systems through alignment between LLM outputs and human preferences. The potential for further applications of LLMs is vast, enabling more flexible and realistic solutions in various fields. For details, please refer to the Appendix~\ref{app:futurework}.

% For detailed discussions and specific recommendations, please refer to the appendix~\ref{app:diss} and \ref{app:futurework}.
